The many faces of degeneracy in conic optimization

Slater's condition -- existence of a "strictly feasible solution" -- is a common assumption in conic optimization. Without strict feasibility, first-order optimality conditions may be meaningless, the dual problem may yield little information about the primal, and small changes in the data may render the problem infeasible. Hence, failure of strict feasibility can negatively impact off-the-shelf numerical methods, such as primal-dual interior point methods, in particular. New optimization modelling techniques and convex relaxations for hard nonconvex problems have shown that the loss of strict feasibility is a more pronounced phenomenon than has previously been realized. In this text, we describe various reasons for the loss of strict feasibility, whether due to poor modelling choices or (more interestingly) rich underlying structure, and discuss ways to cope with it and, in many pronounced cases, how to use it as an advantage. In large part, we emphasize the facial reduction preprocessing technique due to its mathematical elegance, geometric transparency, and computational potential.

==> frontmatter.tex <==
%% Front matter for for FnT Optimization
%% (c) 2013 Neal Parikh (Stanford University)
%% 
%% Based on earlier NOW style files by S. Kumar,
%% J. Sebastian, T. Hoekwater, and B.V. Elvenkind
%%
%% Version 1.01 2014-03-19 Dimitri P. Bertsekas (MIT) 
%% added to EB.
%% Modified by M. Casey

\RequirePackage{lastpage}
\RequirePackage{multicol}

% base journal information definitions
\def\doi#1{\def\@doi{#1}}
\def\copyrightowner#1{\def\@copyrightowner{#1}}
\def\firstpage#1{\def\@firstpage{#1}}
\def\isbn#1{\def\@isbn{#1}}
\def\issue#1{\def\@issue{#1}}
\def\journalinfofont{\fontsize{8}{10}\selectfont\rmfamily}
\def\journallibraryinfo#1{\def\@libraryinfo{#1}}
\def\journaltitle#1{\def\@journaltitle{#1}}
\def\journaltitleprefix#1{\def\@journaltitleprefix{#1}}
\def\@lastpage{\pageref{LastPage}}
\def\lastpage#1{\def\@lastpage{#1}}
\def\copyrightyear#1{\def\@copyrightyear{#1}}
\edef\@copyrightyear{\the\year}
\def\pubyear#1{\def\@pubyear{#1}}
\edef\@pubyear{\the\year}
\def\volume#1{\def\@volume{#1}}

\def\journaltopicintro#1{\def\@journaltopicintro{#1}}
\def\journaltopics#1{\def\@journaltopics{#1}}

% editors
\newcount\editorcount
\def\@editors{}
\def\journaleditor#1{%
  \advance\editorcount1 
  \ifx\empty\@editors
    \def\@editors{#1}%
  \else
    \expandafter\def\expandafter\@editors\expandafter{\@editors\\[0.3em]#1}%
  \fi
}

% editors in chief
\newcount\chiefeditorcount
\def\@chiefeditors{}
\def\journalchiefeditor#1{%
  \advance\chiefeditorcount1 
  \ifx\empty\@chiefeditors
    \def\@chiefeditors{#1}%
  \else
    \expandafter\def\expandafter\@chiefeditors\expandafter{\@chiefeditors\\[0.3em]#1}%
  \fi
}

%% title page

\renewcommand\maketitle{\begin{titlepage}%

\if@openright % -- for 'book' version
\parindent \z@

% title page
\thispagestyle{empty}
\vspace*{\fill}
\begin{flushright}
\begin{minipage}{0.8\textwidth}
\begin{flushright}
\renewcommand{\baselinestretch}{1.1}
\sffamily\bfseries\huge 
\@title
\end{flushright}
\end{minipage}
\end{flushright}
\vspace*{\fill}

% title+author page
\cleardoublepage
\thispagestyle{empty}

\begin{flushright}
{\renewcommand{\baselinestretch}{1.2}
\sffamily\Huge\bfseries \@title\par}
\vspace{3ex}
\noindent\rule{\textwidth}{2pt}
\vspace{1ex}\par

\begingroup
\def\and{%
  \end{tabular}%
  \par\vspace*{2ex}
  \begin{tabular}[t]{r@{}}
  \bfseries}

\Large\sffamily
\begin{tabular}[t]{r@{}}
    \bfseries
    \@author
\end{tabular}
\endgroup
\vfill
\includegraphics[width=53bp]{now_logo}\\
\includegraphics[width=81bp]{essence_logo}\\
Boston --- Delft
\end{flushright}

% publisher page
\newpage
\thispagestyle{empty}
\begingroup

\parskip6pt

{\bfseries\sffamily\Large \@journaltitleprefix\ \@journaltitle}
\footnotesize

\vfill

{\itshape Published, sold and distributed by:}\\
now Publishers Inc.\\
PO Box 1024\\
Hanover, MA\ 02339\\
United States\\
Tel.\ +1-781-985-4510\\
www.nowpublishers.com\\
sales@nowpublishers.com

{\itshape Outside North America:}\\
now Publishers Inc.\\
PO Box 179\\
2600 AD Delft\\
The Netherlands\\
Tel.\ +31-6-51115274

The preferred citation for this publication is

{\raggedright
\@copyrightowner. \emph{\@title}.  \@journaltitleprefix\
\@journaltitle, vol.~\@volume, no.~\@issue, pp.~\@firstpage--\@lastpage,
\@pubyear.\par}

{\itshape This Foundations and Trends\textsuperscript{\textregistered} issue
was typeset in \LaTeX\ using a class file designed by Neal Parikh. Printed on
acid-free paper.}

ISBN: \@isbn\\ \copyright\ \@copyrightyear\ \@copyrightowner

\vfill

\fontsize{8}{9}\selectfont
All rights reserved. No part of this publication may be
reproduced, stored in a retrieval system, or transmitted in any form
or by any means, mechanical, photocopying, recording or otherwise,
without prior written permission of the publishers.

Photocopying. In the USA: This journal is registered at the Copyright
Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923. 
Authorization to photocopy items for
internal or personal use, or the internal or personal use of specific
clients, is granted by now Publishers Inc for users registered with 
the Copyright Clearance Center (CCC).
The `services' for users can be found on the internet at:
www.copyright.com

For those organizations that have been granted a photocopy license, a
separate system of payment has been arranged. Authorization does not
extend to other kinds of copying, such as that for general
distribution, for advertising or promotional purposes, for creating
new collective works, or for resale.  In the rest of the world:
Permission to photocopy must be obtained from the copyright
owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA
02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com;
sales@nowpublishers.com

now Publishers Inc. has an exclusive license to publish this
material worldwide. Permission to use this content must be obtained from
the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
sales@nowpublishers.com\par
\endgroup

% editorial board
\newpage
\thispagestyle{empty}
\begin{center}
\sffamily\LARGE
{\bfseries \@journaltitleprefix\ \@journaltitle}\\
{Volume \@volume, Issue \@issue, \@pubyear}\\
{\bfseries Editorial Board}
\end{center}

\vspace{12pt}

\ifnum\chiefeditorcount>1
{\sffamily\bfseries Editors-in-Chief}
{\footnotesize
\begin{multicols}{2}
\@chiefeditors
\end{multicols}}
\else
{\sffamily\bfseries Editor-in-Chief}\par
\vspace*{10pt}
\begin{footnotesize}
\begin{tabular}[t]{@{}l}
\@chiefeditors \\
\end{tabular}
\end{footnotesize}
\vspace*{10pt}
\fi

{\sffamily \bfseries Editors}
{\footnotesize
\begin{multicols}{2}
\@editors
\end{multicols}}%

% editorial scope
\newpage % page vi -- blank
\thispagestyle{empty}
\begin{center}
{\sffamily\bfseries\LARGE Editorial Scope}
\end{center}

\vspace{18pt}

{\bfseries\large\sffamily Topics}\\

\@journaltopicintro

\fontsize{10}{13}\selectfont
{\raggedright \@journaltopics}

{\bfseries\large\sffamily Information for Librarians}\\

\@libraryinfo\par

\else\fi % -- no book front matter for "journal" version

% -- end book front matter

% title+author page
\newpage
\thispagestyle{empty}
\hbox to \textwidth{%
    \vbox{\raggedright
    \hsize=.6\textwidth \journalinfofont
{\hangindent=3.5ex
\hangafter=1
\@journaltitleprefix\ \@journaltitle\par}%
Vol.~\@volume, No.~\@issue\ (\@pubyear) 
\@firstpage--\@lastpage\\
{\hangindent=3.5ex
\hangafter=1
\copyright\ \@copyrightyear\ \@copyrightowner\par}%
DOI: \@doi}\hss
\vbox{\hsize=.4\textwidth 
    \raggedleft
    \includegraphics[width=53bp]{now_logo}\\
    \includegraphics[width=81bp]{essence_logo}\\
    \par
}}\par
\let\footnoterule\relax
\let\footnote\thanks
\null\vfil
\vskip 60\p@
\begin{center}%
{\LARGE \sffamily \bfseries \@title \par}%
\vskip 3em%
{
\large
\lineskip .75em%
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
\end{center}\par
\@thanks
\vfill
\end{titlepage}
\setcounter{footnote}{0}%
}

%% defaults and settings for this FnT

\def\@copyrightowner{now Publishers Inc.}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\volume{XX}
\issue{XX}
\firstpage{1}
\isbn{XXX-X-XXXXX-XXX-X}
\doi{10.1561/XXXXXXXXXX}

\journaltitle{Optimization}

\journalchiefeditor{\textbf{Stephen Boyd} \\
Stanford University \\
United States}

\journalchiefeditor{\textbf{Yinyu Ye} \\
Stanford University \\
United States}

\journaleditor{Dimitris Bertsimas \\ \emph{Massachusetts Institute of Technology}}
\journaleditor{Dimitri P. Bertsekas \\ \emph{Massachusetts Institute of Technology}}
\journaleditor{John R. Birge \\ \emph{University of Chicago}}
\journaleditor{Robert E. Bixby \\ \emph{Rice University}}
\journaleditor{Emmanuel Cand\`{e}s \\ \emph{Stanford University}}
\journaleditor{David Donoho \\ \emph{Stanford University}}
\journaleditor{Laurent El Ghaoui \\ \emph{University of California, Berkeley}}
\journaleditor{Donald Goldfarb \\ \emph{Columbia University}}
\journaleditor{Michael I. Jordan \\ \emph{University of California, Berkeley}}
\journaleditor{Zhi-Quan (Tom) Luo \\ \emph{University of Minnesota, Twin Cites}}
\journaleditor{George L. Nemhauser \\ \emph{Georgia Institute of Technology}}
\journaleditor{Arkadi Nemirovski \\ \emph{Georgia Institute of Technology}}
\journaleditor{Yurii Nesterov \\ \emph{UC Louvain}}
\journaleditor{Jorge Nocedal \\ \emph{Northwestern University}}
\journaleditor{Pablo A. Parrilo \\ \emph{Massachusetts Institute of Technology}}
\journaleditor{Boris T. Polyak \\ \emph{Institute for Control Science, Moscow}}
\journaleditor{Tam\'{a}s Terlaky \\ \emph{Lehigh University}}
\journaleditor{Michael J. Todd \\ \emph{Cornell University}}
\journaleditor{Kim-Chuan Toh \\ \emph{National University of Singapore}}
\journaleditor{John N. Tsitsiklis \\ \emph{Massachusetts Institute of Technology}}
\journaleditor{Lieven Vandenberghe \\ \emph{University of California, Los Angeles}}
\journaleditor{Robert J. Vanderbei \\ \emph{Princeton University}}
\journaleditor{Stephen J. Wright \\ \emph{University of Wisconsin}}

\journaltopicintro{\@journaltitleprefix\ \@journaltitle\ publishes
survey and tutorial articles on methods for and applications of mathematical optimization, including the following topics:}

\journaltopics{
\begin{itemize}
\item{Algorithm design, analysis, and implementation (especially on
modern computing platforms)}
\item{Models and modeling systems} 
\item{New optimization formulations for practical problems}
\item{Applications of optimization in:}
	\begin{itemize}
	\item Machine learning
	\item Statistics
	\item Data analysis
	\item Signal and image processing
	\item Computational economics and finance
	\item Engineering design
	\item Scheduling and resource allocation
	\item and other areas
	\end{itemize}
\end{itemize}
}

\journallibraryinfo{%
  Foundations and Trends\textsuperscript{\textregistered} in \@journaltitle, \@pubyear,
  Volume~\@volume, 4 issues. ISSN paper version 2167-3888.
  ISSN online version 2167-3918.
  Also available as a combined paper and online
  subscription.
}

\endinput

